NuSTAR view of the central region of M 31

Our neighbouring large spiral galaxy, the Andromeda galaxy (M 31 or NGC 224), is an ideal target to study the X-ray source population of a nearby galaxy. NuSTAR observed the central region of M 31 in 2015 and allows studying the population of X-ray point sources at energies higher than 10 keV. Based on the source catalogue of the large XMM-Newton survey of M 31, we identified counterparts to the XMM-Newton sources in the NuSTAR data. The NuSTAR data only contain sources of a brightness comparable (or even brighter) than the selected sources that have been detected in XMM-Newton data. We investigate hardness ratios, spectra and long-term light curves of individual sources obtained from NuSTAR data. Based on our spectral studies we suggest four sources as possible X-ray binary candidates. The long-term light curves of seven sources that have been observed more than once show low (but significant) variability.

==> spec_par2.tex <==
\addtocounter{table}{-1}
\begin{landscape}
\begin{center}
\begin{longtable}{rrllllllllll}
\tiny
\caption{\label{Tab:Spec_par}Spectral parameters obtained by fitting the \nus\ spectra. Luminosities in units of $10^{36}$ erg/s.}
\hline\noalign{\smallskip}
\multicolumn{1}{c}{src.} &  \multicolumn{1}{c}{obs.} &  \multicolumn{1}{c}{$\Gamma$} & \multicolumn{1}{c}{N$_{\mr{pl}}$} & \multicolumn{1}{c}{C$_{\mr{FPMB; pl}}$} & \multicolumn{1}{c}{T$_{\mr{in}}$ [keV]} &  \multicolumn{1}{c}{N$_{\mr{dbb}}$} & \multicolumn{1}{c}{C$_{\mr{FPMB; dbb}}$} & \multicolumn{1}{c}{T$_{\mr{0}}$ [keV]} & \multicolumn{1}{c}{T$_{\mr{e}}$ [keV]} & \multicolumn{1}{c}{$\tau$}&  \multicolumn{1}{c}{N$_{\mr{ctt}}$} \\
& & \multicolumn{1}{c}{C$_{\mr{FPMB; ctt}}$} &  \multicolumn{1}{c}{$\chi^2_{\mr{pl}}/dof$}  &  \multicolumn{1}{c}{$\chi^2_{\mr{dbb}}/dof$}  &  \multicolumn{1}{c}{$\chi^2_{\mr{ctt}}/dof$}  &  \multicolumn{1}{c}{$L_{\mr{pl}}$} &  \multicolumn{1}{c}{$L_{\mr{dbb}}$} &  \multicolumn{1}{c}{$L_{\mr{ctt}}$} & & &\\
\hline\noalign{\smallskip}
\endfirsthead

\hline\noalign{\smallskip}
\multicolumn{1}{c}{src.} &  \multicolumn{1}{c}{obs.} &  \multicolumn{1}{c}{$\Gamma$} & \multicolumn{1}{c}{N$_{\mr{pl}}$} & \multicolumn{1}{c}{C$_{\mr{FPMB; pl}}$} & \multicolumn{1}{c}{T$_{\mr{in}}$ [keV]} &  \multicolumn{1}{c}{N$_{\mr{dbb}}$} & \multicolumn{1}{c}{C$_{\mr{FPMB; dbb}}$} & \multicolumn{1}{c}{T$_{\mr{0}}$ [keV]} & \multicolumn{1}{c}{T$_{\mr{e}}$ [keV]} & \multicolumn{1}{c}{$\tau$}&  \multicolumn{1}{c}{N$_{\mr{ctt}}$} \\
& & \multicolumn{1}{c}{C$_{\mr{FPMB; ctt}}$} &  \multicolumn{1}{c}{$\chi^2_{\mr{pl}}/dof$}  &  \multicolumn{1}{c}{$\chi^2_{\mr{dbb}}/dof$}  &  \multicolumn{1}{c}{$\chi^2_{\mr{ctt}}/dof$}  &  \multicolumn{1}{c}{$L_{\mr{pl}}$} &  \multicolumn{1}{c}{$L_{\mr{dbb}}$} &  \multicolumn{1}{c}{$L_{\mr{ctt}}$} & & &\\
\hline\noalign{\smallskip}
\endhead

\hline\noalign{\smallskip}
\endfoot

\hline\noalign{\smallskip}
\endlastfoot

 823&6 & $2.40_{-0.24}^{+0.25} $ &$3.51_{-1.29}^{+2.00}E-04 $ &$0.86_{-0.15}^{+0.19} $ &$2.40_{-0.33}^{+0.41} $ &$8.70_{-4.24}^{+7.95}E-04 $ &$0.87_{-0.16}^{+0.19} $ &$4.76_{-4.76}^{+4.53}E-01 $ &$2.89_{-0.97}^{+84.01} $ &$ 5.52_{-5.52}^{+4.48} $ &$6.12_{-6.12}^{+329.60}E-05 $ \\
 & &$0.86_{-0.16}^{+0.19} $ &60.15/58& 61.02 /58& 58.24/56& $3.78_{-0.37}^{+0.37} $ &$	2.37_{-0.23}^{+0.23} $ &$	2.61_{-0.26}^{+0.26} $ & & & \\ 
 855& 6& $ 2.39_{-0.18}^{+0.19} $ &$ 3.86_{-1.16}^{+1.64}E-04 $ &$ 0.94_{-0.15}^{+0.18}$ & $ 2.80_{-0.34}^{+0.40}$ & $ 5.42_{-2.30}^{+3.91}E-04$ & $ 0.91_{-0.15}^{+0.17}$ & $ 2.02_{-2.02}^{+6.47}E-03$ & $ 3.31_{-0.35}^{+0.39}$ & $ 5.30_{-0.56}^{+0.66} $ & $ 8.00_{-0.71}^{+538020.00}E-03$\\
&  & $ 0.92_{-0.15}^{+0.17}$ & 31.79/ 33& 28.27/ 33& 24.73/ 31& $4.33_{-0.37}^{+0.37} $ &$	2.96_{-0.25}^{+0.25} $ &$	3.22_{-0.28}^{+0.28} $ & & & \\
 870&6 & $2.45_{-0.14}^{+0.15} $ &$4.27_{-1.00}^{+1.29}E-04 $ &$1.10_{-0.13}^{+0.15} $ &$2.40_{-0.20}^{+0.22} $ &$1.06_{-0.34}^{+0.48}E-03 $ &$1.02_{-0.12}^{+0.14} $ &$1.43_{-1.43}^{+10.04}E-01 $ &$2.14_{-0.38}^{+0.67} $ &$8.12_{-2.44}^{+4.43} $ &$2.00_{-0.19}^{+1668.80}E-03 $\\
&  &$1.03_{-0.13}^{+0.15} $ &105.80/79 &87.77/79& 87.47/77& $4.16_{-0.27}^{+0.27} $ &$	2.89_{-0.18}^{+0.18} $ &$	2.91_{-0.19}^{+0.19} $ & & & \\ 
 876& 6& $ 2.06_{-0.26}^{+0.28} $ &$ 1.28_{-0.56}^{+0.99}E-04 $ &$ 0.95_{-0.20}^{+0.26}$ & $ 3.79 _{-0.76}^{+1.02}$ & $ 9.33_{-5.68}^{+13.90}E-05$ & $ 0.98_{-0.21}^{+0.27}$ & $ 4.64_{-4.64}^{+5.19}E-01$ & $ 5.99_{-2.75}^{+160.50 }$ & $ 3.86_{-3.80}^{+3.00} $ & $ 1.71_{-1.71}^{+59.76}E-05$\\
&  & $ 0.95_{-0.20}^{+0.26}$ & 21.81/ 24& 26.74/ 24& 21.17/ 22& $3.26_{-0.37}^{+0.37} $ &$	1.93_{-0.22}^{+0.22} $ &$	2.42_{-0.28}^{+0.28} $ & & & \\
 877&6& $2.35_{-0.21}^{+0.23} $ &$2.80_{-0.94}^{+1.39}E-04 $ &$1.03_{-0.18}^{+0.22} $ &$2.69_{-0.36}^{+0.44} $ &$4.83_{-2.22}^{+3.98}E-04 $ &$1.01_{-0.18}^{+0.21} $ &$9.95_{-9.95}^{+1006.89}E-03 $ &$3.26_{-1.03}^{+7.42} $ &$5.26_{-3.09}^{+3.27} $ &$1.66_{-1.66}^{+0.30}E-03 $ \\
& &$1.02_{-0.18}^{+0.21} $ &82.51/74& 81.92/74 &78.62/72 &$3.40_{-0.32}^{+0.32} $ &$	2.23_{-0.21}^{+0.21} $ &$	2.43_{-0.23}^{+0.23} $  & & & \\ 
 910& 6& $ 2.52_{-0.25}^{+0.26} $ &$ 2.58_{-0.98}^{+1.56}E-04 $ &$ 1.10_{-0.21}^{+0.27}$ & $ 2.33 _{-0.32}^{+0.39}$ & $ 6.19_{-3.00}^{+5.64}E-04$ & $ 1.10_{-0.21}^{+0.26}$ & $ 3.40_{-3.30}^{+10.14}E-01$ & $ 2.08_{-0.56}^{+1.37}$ & $ 8.22_{-3.81}^{+10.60 } $ & $ 5.72_{-5.72}^{+96.84}E-05$ \\
& & $ 1.10_{-0.21}^{+0.26}$ & 77.37/ 58& 69.02/ 58& 68.71/ 56& $2.14_{-0.23}^{+0.23} $ &$	1.48_{-0.16}^{+0.16} $ &$	1.50_{-0.16}^{+0.16} $  & & & \\
 911&6 & $2.20_{-0.24}^{+0.25} $ &$1.54_{-0.56}^{+0.87}E-04 $ &$1.03_{-0.19}^{+0.24} $ &$2.90_{-0.44}^{+0.55} $ &$2.51_{-1.25}^{+2.41}E-04 $ &$1.08_{-0.20}^{+0.25} $ &$3.83_{-3.83}^{+4.07}E-01 $ &$3.47_{-1.11}^{+124.13 } $ &$5.32_{-5.17}^{+3.07} $ &$3.43_{-3.43}^{+101.60} E-05$ \\
& &$1.06_{-0.20}^{+0.24} $ &67.17/72& 70.03/72& 65.65/70 & $2.74_{-0.28}^{+0.28} $ &$	1.62_{-0.17}^{+0.17} $ &$	1.80_{-0.18}^{+0.18} $  & & & \\ 
 922& 6& $ 2.42_{-0.10}^{+0.11} $ &$ 7.06_{-1.29}^{+1.56}E-04 $ &$ 1.04_{-0.10}^{+0.11}$ & $ 2.53 _{-0.16}^{+0.18}$ & $ 1.44_{-0.37}^{+0.49}E-03$ & $ 1.05_{-0.10}^{+0.11}$ & $ 7.09_{-7.09}^{+3.33}E-01$ & $ 2.42_{-0.43}^{+1.42}$ & $ 6.98_{-3.30}^{+2.97} $ & $ 9.69_{-4.46}^{+160.59}E-05$ \\
& & $ 1.05_{-0.10}^{+0.11}$ & 156.74/ 114& 118.86/ 114& 117.50/ 112& $7.40_{-0.38}^{+0.38} $ &$	4.99_{-0.25}^{+0.25} $ &$	5.10_{-0.26}^{+0.26} $ & & & \\
 930& 6& $ 1.22_{-0.04}^{+0.04} $ &$ 1.37_{-0.13}^{+0.15}E-04 $ &$ 1.13_{-0.06}^{+0.06}$ & $ 10.48_{-0.75}^{+0.84}$ & $ 1.94_{-0.41}^{+0.51}E-05$ & $ 1.17_{-0.06}^{+0.06}$ & $ 1.02_{-1.02}^{+0.03}E-03$ & $ 198.37 _{-198.37 }^{+65.13}$ & $ 1.08_{-0.69}^{+0.28} $ & $ 1.18_{-0.03}^{+1.29}E-05$ \\
& & $ 1.14_{-0.06}^{+0.06}$ & 321.52/ 246& 256.18/ 246& 316.76/ 244& $45.20_{-1.23}^{+1.23} $ &$	27.30_{-0.73}^{+0.74} $ &$	44.20_{-1.20}^{+1.20} $ & & & \\
 966& 6& $ 3.01_{-0.04}^{+0.04} $ &$ 8.82_{-0.67}^{+0.73}E-03 $ &$ 0.93_{-0.04}^{+0.04}$ & $ 1.87 _{-0.04}^{+0.04}$ & $ 2.48_{-0.26}^{+0.29}E-02$ & $ 0.94_{-0.04}^{+0.04}$ & $ 6.24_{-6.24}^{+1.40}E-01$ & $ 2.04_{-0.21}^{+0.35}$ & $ 6.26_{-1.37}^{+1.22} $ & $ 7.90_{-1.99}^{+230.01}E-04$ \\
& & $ 0.93_{-0.04}^{+0.04}$ & 513.82/ 290& 301.08/ 290& 277.06/ 288& $25.70_{-0.53}^{+0.53} $ &$	20.90_{-0.42}^{+0.42} $ &$	21.60_{-0.44}^{+0.44} $ & & & \\
 972& 6& $ 1.77_{-0.47}^{+0.52} $ &$ 3.86_{-2.44}^{+6.27}E-05 $ &$ 1.02_{-0.34}^{+0.53}$ & $ 4.72 _{-1.88}^{+4.33}$ & $ 2.29_{-2.29}^{+12.76}E-05$ & $ 0.98_{-0.34}^{+0.51}$ & $ 5.34_{-5.34}^{+8.95}E-01$ & $ 6.68_{-3.78}^{+110.62 }$ & $ 4.33_{-4.33}^{+4.61} $ & $ 6.21_{-6.21}^{+186.17}E-06$ \\
& & $ 1.01_{-0.34}^{+0.52}$ & 51.82/ 41& 53.38/ 41& 51.29/ 39& $2.21_{-0.44}^{+0.44} $ &$	1.20_{-0.24}^{+0.24} $ &$	1.55_{-0.31}^{+0.31} $  & & & \\
1015&4 & $2.47_{-0.31}^{+0.34} $ &$1.18_{-0.53}^{+0.96}E-03 $ &$0.79_{-0.20}^{+0.24} $ &$2.38_{-0.43}^{+0.55} $ &$2.63_{-1.54}^{+3.58}E-03 $ &$0.81_{-0.21}^{+0.24} $ &$1.25_{-1.25}^{+8.84}E-01 $ &$250.00_{-244.57}^{+143.26} $ &$0.01_{-0.01}^{+3.81} $ &$1.59_{-1.59}^{+96.12}E-01 $ \\
& &$0.79_{-0.20}^{+0.24} $ &26.38/35& 30.64/35 &26.39/33&  $10.80_{-1.33}^{+1.33} $ &$	6.97_{-0.87}^{+0.87} $ &$	10.60_{-1.31}^{+1.31} $  & & & \\
1015&5 & $2.65_{-0.23}^{+0.25} $ &$1.72_{-0.61}^{+0.94}E-03 $ &$1.04_{-0.20}^{+0.24} $ &$2.07_{-0.27}^{+0.32} $ &$5.38_{-2.56}^{+4.68}E-03 $ &$1.00_{-0.20}^{+0.23} $ &$7.45_{-7.44}^{+2.59}E-01 $ &$13.47_{-12.46}^{+188.90} $ &$1.06_{-1.06}^{+5.99} $ &$2.99_{-2.99}^{+194.70}E-05 $ \\
& &$1.02_{-0.20}^{+0.23} $ &67.45/ 47 &69.18/47 &64.62/45& $  10.60_{-1.04}^{+1.04} $ &$	7.45_{-0.74}^{+0.74} $ &$	9.12_{-0.89}^{+0.89} $  & & & \\ 
1015&6 & $2.60_{-0.07}^{+0.07} $ &$2.31_{-0.27}^{+0.31}E-03 $ &$0.96_{-0.06}^{+0.06} $ &$2.28_{-0.09}^{+0.10} $ &$5.12_{-0.87}^{+1.04}E-03 $ &$0.98_{-0.06}^{+0.06} $ &$3.21_{-3.21}^{+2.51}E-01 $ &$ 3.16 _{-0.50}^{+ 0.81} $ &$4.74_{-0.89}^{+0.92} $ &$4.64_{-2.32}^{+229.95}E-04 $ \\
& &$0.97_{-0.06}^{+0.06} $ &201.09/178 &210.65/178 &168.86/176 &$ 15.80_{-0.47}^{+0.47} $ &$	11.20_{-0.33}^{+0.33} $ &$	12.40_{-0.37}^{+0.37} $ & & & \\
1024 &  4 & $ 2.66_{-0.29}^{+ 0.31} $ &$  1.54_{-0.62}^{+1.05}E-03 $ &$0.92_{-0.19}^{+0.23} $ &$1.98_{-0.30}^{+0.37} $ &$5.60_{-2.99}^{+6.16}E-03 $ &$0.91_{-0.19}^{+0.23} $ &$ 5.83_{-5.83}^{+ 2.86}E-01 $ &$ 175.75_{- 174.75}^{+ 93.86} $ &$0.01_{-0.01}^{+3.84} $ &$2.54_{-1.12}^{+849.00}E-06 $ \\
& &$ 0.92_{-0.19}^{+0.22} $ & 53.28/45  &  59.76/45 &53.062/ 43 &$ 9.23_{-1.00}^{+1.00} $ &$	6.32_{-0.70}^{+0.70} $ &$	8.80_{-0.96}^{+0.96} $  & & & \\
1024 &  5 & $ 2.69_{-0.23}^{+0.24} $ &$1.70_{-0.59}^{+0.91}E-03 $ &$0.95_{-0.16}^{+0.19} $ &$2.04_{-0.26}^{+0.31} $ &$5.15_{-2.45}^{+4.49}E-03 $ &$0.93_{-0.16}^{+0.19} $ &$1.26_{-  1.26}^{+  807.87}E-03  $ &$22.72_{-22.72}^{+4.93} $ &$0.65_{-0.14}^{+5.46} $ &$3.26_{-0.29}^{+31.43}E-01 $ \\
& &$0.95_{-0.16}^{+0.19} $ & 48.58/60  &  59.16/60  &  48.44/58 &$  9.48_{-0.85}^{+0.85} $ &$	6.63_{-0.60}^{+0.60} $ &$	8.95_{-0.80}^{+0.80} $& & & \\
1024&6 & $2.61_{-0.07}^{+0.07} $ &$1.97_{-0.26}^{+0.29}E-03 $ &$1.06_{-0.07}^{+0.07} $ &$2.23_{-0.10}^{+0.10} $ &$4.77_{-0.88}^{+1.07}E-03 $ &$1.08_{-0.07}^{+0.07} $ &$2.90_{-2.90}^{+869.0}E-03 $ &$ 2.89 _{- 0.12}^{+0.12} $ &$5.09_{-0.20}^{+0.22} $ &$6.55_{-0.22}^{+36.20}E-02 $ \\
& &$1.07_{-0.07}^{+0.07} $ &171.94/160 &166.93/160 &142.95/158 & $13.30_{-0.44}^{+0.44} $ &$	9.35_{-0.31}^{+0.31} $ &$	10.20_{-0.34}^{+0.34} $  & & & \\
1036& 1& $ 2.52_{-0.13}^{+0.14} $ &$ 1.16_{-0.28}^{+0.36}E-03 $ &$ 1.20_{-0.14}^{+0.17}$ & $ 2.40 _{-0.18}^{+0.20}$ & $ 2.46_{-0.74}^{+1.05}E-03$ & $ 1.18_{-0.14}^{+0.16}$ & $ 3.46_{-3.46}^{+6.20}E-01$ & $ 2.05_{-0.32}^{+0.51}$ & $ 8.74_{-2.54}^{+4.88} $ & $ 2.37_{-1.20}^{+23.64}E-04$ \\
& & $ 1.17_{-0.14}^{+0.16}$ & 108.43/ 89& 85.44/ 89& 84.83/ 87& $9.54_{-0.60}^{+0.60} $ &$	6.75_{-0.42}^{+0.42} $ &$	6.77_{-0.42}^{+0.42} $ & & & \\
1036& 4& $ 2.29_{-0.35}^{+0.38} $ &$ 6.84_{-3.40}^{+6.57}E-04 $ &$ 1.00_{-0.41}^{+0.50}$ & $ 2.58 _{-0.48}^{+0.67}$ & $ 1.61_{-1.00}^{+2.28}E-03$ & $ 0.94_{-0.38}^{+0.45}$ & $ 4.38_{-1.42}^{+7.85}$ & $ 1.00_{-1.00}^{+0.00}$ & $ 72.54_{-44.21}^{+104.84} $ & $ 2.20_{-1.00}^{+23.70}E-03$ \\
& & $ 0.86_{-0.34}^{+0.39}$ & 30.33/ 18& 24.32/ 18& 18.54/ 16& $9.68_{-1.52}^{+1.52} $ &$	6.12_{-0.94}^{+0.94} $ &$	6.81_{-1.02}^{+1.02} $  & & & \\
1036& 5& $ 2.42_{-0.26}^{+0.28} $ &$ 9.97_{-3.88}^{+6.24}E-04 $ &$ 0.59_{-0.19}^{+0.21}$ & $ 2.45 _{-0.36}^{+0.46}$ & $ 2.30_{-1.18}^{+2.26}E-03$ & $ 0.61_{-0.18}^{+0.21}$ & $ <1.00E-03$ & $ 2.24_{-0.69}^{+0.32}$ & $ 7.70_{-3.99}^{+1.91} $ & $ 1.60_{-0.19}^{+20.13}E-02$ \\
& & $ 0.61_{-0.18}^{+0.21}$ & 20.71/ 30& 14.75/ 30& 14.75/ 28& $10.40_{-1.25}^{+1.25} $ &$	6.87_{-0.81}^{+0.81} $ &$	7.00_{-0.83}^{+0.83} $  & & & \\
1036&6 & $2.61_{-0.10}^{+0.10} $ &$1.28_{-0.22}^{+0.26}E-03 $ &$0.94_{-0.08}^{+0.09} $ &$2.17_{-0.12}^{+0.14} $ &$3.58_{-0.86}^{+1.11} E-03$ &$0.92_{-0.08}^{+0.09} $ &$8.84_{-1.86}^{+1.24}E-01 $ &$5.85_{-3.13}^{+132.78} $ &$2.28_{-2.23}^{+2.81} $ &$4.92_{-4.92}^{+7.79}E-05 $ \\
& &$0.92_{-0.08}^{+0.09} $ &147.20/114& 134.02/114 &122.94/112 & $8.58_{-0.39}^{+0.39} $ &$	6.14_{-0.28}^{+0.28} $ &$	6.88_{-0.31}^{+0.31} $  & & & \\
1060& 3& $ 2.28_{-0.26}^{+0.27} $ &$ 2.60_{-1.06}^{+1.73}E-04 $ &$ 1.49_{-0.32}^{+0.44}$ & $ 2.70 _{-0.40}^{+0.50}$ & $ 4.94_{-2.50}^{+4.88}E-04$ & $ 1.60_{-0.34}^{+0.47}$ & $ 2.87_{-2.87}^{+39.39}E-01$ & $ 2.08_{-0.42}^{+21.46}$ & $ 10.56_{-4.46}^{+180.26} $ & $ 6.16_{-3.36}^{+40.81}E-05$ \\
& & $ 1.61_{-0.34}^{+0.48}$ & 107.87/ 83& 96.86/ 83& 96.07/ 81& $3.79_{-0.46}^{+0.46} $ &$	2.32_{-0.27}^{+0.27} $ &$	2.25_{-0.26}^{+0.26} $ & & & \\
1060& 4& $ 2.36_{-0.28}^{+0.30} $ &$ 5.35_{-2.27}^{+3.86}E-04 $ &$ 0.94_{-0.23}^{+0.28}$ & $ 2.64 _{-0.47}^{+0.61}$ & $ 1.01_{-0.58}^{+1.32}E-03$ & $ 0.92_{-0.22}^{+0.27}$ & $ 7.31_{-7.31}^{+5.16}E-01$ & $ 3.06_{-1.19}^{+97.64}$ & $ 5.45_{-5.31}^{+6.37} $ & $ 6.42_{-6.42}^{+502.78}E-05$ \\
& & $ 0.92_{-0.22}^{+0.27}$ & 27.46/ 35& 24.13/ 35& 22.91/ 33& $6.44_{-0.84}^{+0.84} $ &$	4.23_{-0.54}^{+0.54} $ &$	4.54_{-0.58}^{+0.58} $ & & & \\
1060& 5& $ 2.77_{-0.32}^{+0.35} $ &$ 1.03_{-0.45}^{+0.83}E-03 $ &$ 0.89_{-0.21}^{+0.26}$ & $ 2.07 _{-0.32}^{+0.40}$ & $ 2.53_{-1.38}^{+2.96}E-03$ & $ 0.91_{-0.21}^{+0.26}$ & $ 1.73_{-1.73}^{+1185.13}E-03$ & $ 12.52_{-12.52}^{+3.57}$ & $ 1.24_{-0.30}^{+0.36} $ & $ 3.00_{-0.29}^{+134739.00}E-01$ \\
& & $ 0.89_{-0.21}^{+0.26}$ & 35.84/ 41& 35.37/ 41& 35.27/ 39& $4.83_{-0.60}^{+0.60} $ &$	3.50_{-0.43}^{+0.43} $ &$	4.48_{-0.56}^{+0.56} $ & & & \\
1060& 6& $ 2.44_{-0.18}^{+0.19} $ &$ 6.40_{-1.92}^{+2.73}E-04 $ &$ 0.86_{-0.12}^{+0.14}$ & $ 2.48 _{-0.28}^{+0.33}$ & $ 1.31_{-0.55}^{+0.90}E-03$ & $ 0.85_{-0.12}^{+0.14}$ & $ 3.79_{-3.79}^{+3.18}E-01$ & $ 4.97_{-2.33}^{+246.02 }$ & $ 3.46_{-3.34}^{+2.79} $ & $ 8.72_{-8.72}^{+585.34}E-05$ \\
& & $ 0.86_{-0.12}^{+0.14}$ & 56.79/ 73& 66.10/ 73& 55.99/ 71& $6.32_{-0.49}^{+0.49} $ &$	4.14_{-0.32}^{+0.32} $ &$	5.03_{-0.39}^{+0.39} $ & & & \\
1075&1 & $2.54_{-0.27}^{+0.29} $ &$3.74_{-1.68}^{+2.92}E-04 $ &$1.34_{-0.30}^{+0.43} $ &$2.22_{-0.32}^{+0.41} $ &$1.04_{-0.58}^{+1.20}E-03 $ &$1.34_{-0.30}^{+0.43} $ &$1.00_{-0.48}^{+0.37} $ &$103.36_{-102.32}^{+120.32} $ &$0.01_{-0.01}^{+3.99} $ &$6.85_{-3.52}^{+2505.81}E-07 $ \\
& &$1.35_{-0.30}^{+0.43} $ & 63.95/57 &60.08/57 &59.35/55& $2.92_{-0.35}^{+0.35} $ &$	1.99_{-0.24}^{+0.24} $ &$	2.24_{-0.27}^{+0.27} $ & & & \\ 
1075&4 & $3.26_{-0.55}^{+0.70} $ &$1.29_{-0.80}^{+2.43}E-03 $ &$1.25_{-0.38}^{+0.58} $ &$1.62_{-0.35}^{+0.44} $ &$4.64_{-4.64}^{+10.81}E-03 $ &$1.19_{-0.37}^{+0.55} $ &$2.89_{-2.89}^{+6.04}E-01 $ &$34.63_{-33.62}^{+152.41} $ &$0.20_{-0.20}^{+5.19} $ &$2.10_{-2.16}^{+21678.60}E-05 $ \\
& &$1.25_{-0.38}^{+0.58} $ & 49.40/34 &50.97/34 &49.38/32&$ 2.34_{-0.42}^{+0.42} $ &$	1.95_{-0.35}^{+0.35} $ &$	2.30_{-0.41}^{+0.41} $ & & & \\
1075&5 & $3.25_{-0.50}^{+0.58} $ &$9.93_{-5.99}^{+15.50}E-04 $ &$1.46_{-0.44}^{+0.68} $ &$1.49_{-0.31}^{+0.40} $ &$5.39_{-5.39}^{+12.76}E-03 $ &$1.39_{-0.42}^{+0.64} $ &$6.94 _{-6.94}^{+4.83}E-01 $ &$20.42_{-20.42}^{+147.38} $ &$0.30_{-0.30}^{+9.68} $ &$6.00_{-5.57}^{+172395.00}E-06 $ \\
& &$1.42_{-0.43}^{+0.67} $ & 33.27/44 &33.05/44 &32.45/42& $1.85_{-0.33}^{+0.33} $ &$	1.51_{-0.27}^{+0.27} $ &$	1.66_{-0.29}^{+0.29} $  & & & \\
1075& 6& $ 2.78_{-0.19}^{+0.20} $ &$ 8.05_{-2.44}^{+3.48}E-04 $ &$ 1.00_{-0.15}^{+0.18}$ & $ 1.99 _{-0.19}^{+0.21}$ & $ 2.42_{-0.91}^{+1.43}E-03$ & $ 1.00_{-0.15}^{+0.18}$ & $ 3.79_{-3.79}^{+6.88}E-01$ & $ 1.75_{-0.34}^{+1.74}$ & $ 9.02_{-3.37}^{+8.03} $ & $ 1.39_{-1.39}^{+15.40}E-04$ \\
& & $ 1.00_{-0.15}^{+0.18}$ & 76.10/ 72& 60.88/ 72& 60.46/ 70& $3.75_{-0.31}^{+0.31} $ &$	2.79_{-0.22}^{+0.23} $ &$	2.81_{-0.23}^{+0.23} $  & & & \\
1091&6 & $2.84_{-0.35}^{+0.39} $ &$4.02_{-1.90}^{+3.64}E-04 $ &$1.21_{-0.29}^{+0.39 } $ &$1.89_{-0.29}^{+0.36} $ &$1.34_{-0.73}^{+1.55}E-03 $ &$1.23_{-0.29}^{+0.39} $ &$3.43_{-3.43}^{+11.76}E-01 $ &$1.58_{-0.38}^{+2.63} $ &$10.52_{-6.44}^{+12.99} $ &$6.69_{-3.84}^{+132.44}E-05 $ \\
& &$1.23_{-0.29}^{+0.39} $ &54.14/46 &49.45/46 &49.10/44 &$1.64_{-0.22}^{+0.22} $ &$	1.20_{-0.16}^{+0.16} $ &$	1.20_{-0.16}^{+0.16} $ & & & \\
1102& 1& $ 2.83_{-0.40}^{+0.46} $ &$ 3.52_{-1.87}^{+4.11}E-04 $ &$ 1.32_{-0.36}^{+0.56}$ & $ 1.89 _{-0.36}^{+0.47}$ & $ 1.18_{-0.76}^{+2.11}E-03$ & $ 1.38_{-0.38}^{+0.60}$ & $ 2.90_{-2.90}^{+9.52}E-01$ & $ 2.78_{-1.51}^{+127.98 }$ & $ 4.59_{-1.47}^{+11.84 } $ & $ 7.83_{-7.83}^{+912.31}E-05$ \\
& & $ 1.35_{-0.37}^{+0.58}$ & 42.59/ 51& 42.93/ 51& 42.05/ 49& $1.46_{-0.23}^{+0.23} $ &$	1.05_{-0.17}^{+0.17} $ &$	1.17_{-0.19}^{+0.19} $  & & & \\
1102& 2& $ 2.88_{-0.42}^{+0.48} $ &$ 4.49_{-2.57}^{+6.06}E-04 $ &$ 1.06_{-0.33}^{+0.46}$ & $ 1.97 _{-0.41}^{+0.53}$ & $ 1.16_{-0.79}^{+2.50}E-03$ & $ 1.10_{-0.33}^{+0.47}$ & $ 6.99_{-6.99}^{+9.91}E-01$ & $ 2.23_{-0.96}^{+53.51}$ & $ 5.80_{-5.80}^{+8.42} $ & $ 3.79_{-3.79}^{+1642.73}E-05$ \\
& & $ 1.09_{-0.33}^{+0.47}$ & 82.35/ 54& 79.81/ 54& 79.25/ 52& $1.69_{-0.29}^{+0.28} $ &$	1.26_{-0.21}^{+0.21} $ &$	1.32_{-0.22}^{+0.22} $ & & & \\
1102& 3& $ 2.93_{-0.33}^{+0.37} $ &$ 6.14_{-2.78}^{+5.23}E-04 $ &$ 1.20_{-0.28}^{+0.37}$ & $ 1.88 _{-0.30}^{+0.35}$ & $ 1.78_{-0.99}^{+2.30}E-03$ & $ 1.26_{-0.29}^{+0.39}$ & $ 4.19_{-4.19}^{+4.64}E-01$ & $ 2.00_{-0.59}^{+2.81}$ & $ 6.53_{-3.73}^{+4.62} $ & $ 8.84_{-8.84}^{+587.71}E-05$ \\
& & $ 1.25_{-0.28}^{+0.39}$ & 79.00/ 77& 75.74/ 77& 74.26/ 75& $2.09_{-0.27}^{+0.27} $ &$	1.57_{-0.20}^{+0.20} $ &$	1.65_{-0.21}^{+0.21} $  & & & \\
1102& 4& $ 3.32_{-0.69}^{+0.89} $ &$ 6.97_{-6.97}^{+18.52}E-04 $ &$ 1.51_{-0.64}^{+1.34}$ & $ 1.59 _{-0.45}^{+0.64}$ & $ 2.57_{-2.57}^{+10.44}E-03$ & $ 1.35_{-0.57}^{+1.11}$ & $ 1.03_{-1.03}^{+0.36}$ & $ 17.78_{-17.78}^{+68.29}$ & $ 0.02_{-0.02}^{+61.69 } $ & $ 2.68_{-2.68}^{+62.55}E-06$ \\
& & $ 1.34_{-0.57}^{+1.11}$ & 27.60/ 28& 25.12/ 28& 25.05/ 26& $1.13_{-0.30}^{+0.30} $ &$	1.00_{-0.26}^{+0.26} $ &$	0.97_{-0.25}^{+0.25} $  & & & \\
1102& 5& $ 3.08_{-0.39}^{+0.44} $ &$ 6.46_{-3.38}^{+7.24}E-04 $ &$ 1.64_{-0.46}^{+0.78}$ & $ 1.80 _{-0.29}^{+0.35}$ & $ 1.84_{-1.07}^{+2.55}E-03$ & $ 1.67_{-0.46}^{+0.76}$ & $ 1.31_{-0.17}^{+0.85}$ & $ 1.00_{-1.00}^{+-1.00}$ & $ 0.05_{-0.05}^{+30.02 } $ & $ 9.09_{-1.37}^{+3.69}E-05$ \\
& & $ 1.70_{-0.47}^{+0.77}$ & 73.54/ 42& 64.64/ 42& 64.12/ 40& $1.64_{-0.26}^{+0.26} $ &$	1.31_{-0.20}^{+0.20} $ &$	1.24_{-0.19}^{+0.19} $  & & & \\
1102& 6& $ 2.89_{-0.39}^{+0.43} $ &$ 6.17_{-3.16}^{+6.54}E-04 $ &$ 1.23_{-0.32}^{+0.48}$ & $ 1.86 _{-0.32}^{+0.40}$ & $ 2.03_{-1.22}^{+2.98}E-03$ & $ 1.24_{-0.32}^{+0.48}$ & $ 4.27_{-4.27}^{+8.04}E-01$ & $ 1.89_{-0.62}^{+67.52}$ & $ 7.07_{-6.35}^{+10.15 } $ & $ 9.56_{-9.56}^{+1078.98}E-05$ \\
& & $ 1.24_{-0.32}^{+0.48}$ & 48.45/ 50& 46.81/ 50& 46.20/ 48& $2.27_{-0.34}^{+0.34} $ &$	1.70_{-0.25}^{+0.25} $ &$	1.76_{-0.26}^{+0.26} $ & & & \\
1103&1 & $2.37_{-0.18}^{+0.19} $ &$3.84_{- 1.16}^{+1.64}E-04 $ &$1.02_{- 0.16}^{+0.19} $ &$2.61_{- 0.29}^{+0.33} $ &$7.36_{- 2.93}^{+4.78}E-04 $ &$1.01_{- 0.15}^{+0.18} $ &$5.35 _{-5.35}^{+5.64}E-01 $ &$2.35_{-0.48 }^{+1.30 } $ &$7.82 _{-2.52 }^{+4.66 } $ &$ 6.53_{-3.38}^{+106.35}E-05 $ \\
& &$1.01 _{-0.15 }^{+0.18} $ &75.82/61 &60.35/ 61 &59.65 /59& $4.46_{-0.37}^{+0.37} $ &$	2.96_{-0.24}^{+0.24} $ &$	3.01_{-0.24}^{+0.24} $  & & & \\
1103&2 & $2.63_{-0.20}^{+0.21} $ &$5.69_{- 1.83}^{+2.67}E-04 $ &$1.13_{- 0.19}^{+0.23} $ &$2.11_{- 0.22}^{+0.26} $ &$1.73_{-0.71}^{+1.15}E-03 $ &$1.13_{- 0.18}^{+0.22} $ &$1.06_{-1.06}^{+0.57} $ &$2.56_{-2.56 }^{+95.16} $ &$4.26 _{-4.26 }^{+22.55 } $ &$ 4.88 _{-4.88 }^{+72.59}E-05 $ \\
& &$1.13 _{-0.18 }^{+0.22} $ &68.95/68 &53.18/ 68 &52.75 / 66&$3.65_{-0.33}^{+0.33} $ &$	2.61_{-0.23}^{+0.23} $ &$	2.62_{-0.23}^{+0.23} $ & & & \\
1103&3 & $2.29_{-0.22}^{+0.24} $ &$3.54_{- 1.24}^{+1.92}E-04 $ &$1.05_{- 0.20}^{+0.23} $ &$2.63_{- 0.35}^{+0.43} $ &$7.47_{- 3.50}^{+6.30}E-04 $ &$1.06_{- 0.20}^{+0.23} $ &$9.95_{-9.95}^{+1517.03}E-03 $ &$2.23_{-0.58 }^{+1.79 } $ &$8.51 _{-4.06 }^{+9.68 } $ &$ 8.10_{-8.10}^{+0.84}E-04  $ \\
& &$1.06 _{-0.20 }^{+0.23} $ &76.72/67 &70.48/ 67 &70.46 /65&$5.02_{-0.48}^{+0.49} $ &$	3.10_{-0.30}^{+0.30} $ &$	3.10_{-0.30}^{+0.30} $  & & & \\
1103&4 & $2.50_{-0.23}^{+0.25} $ &$6.03_{- 2.15}^{+3.32}E-04 $ &$1.09_{- 0.20}^{+0.24} $ &$2.39_{- 0.31}^{+0.38} $ &$1.30_{- 0.61}^{+1.10}E-03 $ &$1.12_{- 0.20}^{+0.25} $ &$4.05_{-4.05}^{+5.69}E-01 $ &$2.60_{-0.77 }^{+17.95} $ &$6.09 _{-3.94 }^{+4.52 } $ &$ 1.15_{-1.15}^{+45.18}E-04 $ \\
& &$1.11 _{-0.20 }^{+0.24} $ &28.84 /41& 26.98 /41& 24.99/39&$ 5.24_{-0.51}^{+0.51} $ &$	3.48_{-0.34}^{+0.34} $ &$	3.74_{-0.36}^{+0.36} $ & & & \\ 
1103&5 & $2.36_{-0.19}^{+0.20} $ &$4.36_{- 1.33}^{+1.91}E-04 $ &$1.15_{- 0.18}^{+0.22} $ &$2.64_{- 0.32}^{+0.37} $ &$8.13_{- 3.40}^{+5.76}E-04 $ &$1.12_{- 0.18}^{+0.21} $ &$4.10_{-4.10}^{+4.02}E-01  $ &$3.06_{-0.86 }^{+18.71} $ &$5.55 _{-4.92 }^{+2.94 } $ &$8.54_{- 8.54}^{+308.86}E-05 $ \\
& &$ 1.14_{- 0.18}^{+0.21 } $ &52.58/56 &53.68/ 56 &49.32 /54& $ 5.22_{-0.44}^{+0.44} $ &$	3.45_{-0.29}^{+0.29} $ &$	3.71_{-0.31}^{+0.31} $  & & & \\ 
1103&6 & $2.44_{-0.16}^{+0.17} $ &$5.30_{- 1.44}^{+1.95}E-04 $ &$1.19_{- 0.16}^{+0.20} $ &$2.39_{- 0.22}^{+0.25} $ &$1.29_{- 0.46}^{+0.69}E-03 $ &$1.21_{- 0.16}^{+0.19} $ &$5.17_{-5.17}^{+5.75}E-01 $ &$2.12_{-0.39 }^{+ 3.50} $ &$8.27 _{-3.85 }^{+4.91 } $ &$9.45_{- 9.45}^{+114.00}E-05 $ \\
& &$ 1.21_{- 0.16}^{+0.19 } $ & 96.96/ 80&81.68/80&81.20/78& $ 5.25_{-0.38}^{+0.38} $ &$	3.48_{-0.25}^{+0.25} $ &$	3.53_{-0.25}^{+0.25} $  & & & \\
1116&1 & $2.68_{-0.26}^{+0.28} $ &$4.85_{- 1.80}^{+2.86}E-04 $ &$0.85_{- 0.17}^{+0.20} $ &$2.05_{- 0.27}^{+0.33} $ &$1.52_{- 0.73}^{+1.38}E-03 $ &$0.83_{- 0.16}^{+0.19} $ &$2.79_{-2.79}^{+9.37}E-01 $ &$2.02_{-0.60}^{+44.77 } $ &$7.31 _{-3.56 }^{+9.74 } $ &$1.27_{- 1.27}^{+29.98}E-04 $ \\
& &$ 0.83_{- 0.16}^{+0.20 } $ &45.29/49 &38.90/ 49 &38.48 /47&$2.78_{-0.30}^{+0.30} $ &$	2.02_{-0.21}^{+0.21} $ &$	2.07_{-0.22}^{+0.22} $  & & & \\
1116&2 & $2.78_{-0.17}^{+0.18} $ &$9.27_{- 2.46}^{+3.33}E-04 $ &$1.25_{- 0.16}^{+0.20} $ &$1.94_{- 0.17}^{+0.19} $ &$3.10_{- 1.07}^{+1.62}E-03 $ &$1.26_{- 0.17}^{+0.20} $ &$5.16_{-5.16}^{+4.48}E-01 $ &$2.20_{-0.56}^{+60.94 } $ &$6.13 _{-2.67 }^{+2.46 } $ &$1.25_{- 1.25}^{+79.89}E-04 $ \\
& &$ 1.26_{- 0.16}^{+0.20 } $ &78.22/81 &72.42/ 81 &69.73 /79&$4.34_{-0.30}^{+0.30} $ &$	3.18_{-0.22}^{+0.22} $ &$	3.35_{-0.23}^{+0.23} $  & & & \\
1116&3 & $2.33_{-0.30}^{+0.32} $ &$2.46_{- 1.08}^{+1.89}E-04 $ &$1.09_{- 0.27}^{+0.32} $ &$2.47_{- 0.40}^{+0.52} $ &$6.38_{- 3.51}^{+7.30}E-04 $ &$1.07_{- 0.26}^{+0.32} $ &$1.23_{-1.22}^{+0.72} $ &$52.69_{- 52.69}^{+114.61} $ &$ 0.03 _{-0.03 }^{+4.06 } $ &$1.08_{- 1.08}^{+65.92}E-06 $ \\
& &$ 1.08_{- 0.26}^{+0.32 } $ &56.66/60 &51.87/ 60 &51.93 /58& $3.20_{-0.41}^{+0.41} $ &$	2.00_{-0.25}^{+0.25} $ &$	2.06_{-0.26}^{+0.26} $  & & & \\
1116&4 & $2.30_{-0.29}^{+0.31} $ &$2.81_{- 1.19}^{+2.04}E-04 $ &$1.02_{- 0.24}^{+0.31} $ &$2.63_{- 0.44}^{+0.58} $ &$5.93_{- 3.30}^{+6.88}E-04 $ &$1.01_{- 0.23}^{+0.30} $ &$4.71_{-4.71}^{+13.21}E-01 $ &$2.22 _{- 0.67}^{+32.61} $ &$8.68_{- 8.68}^{+188.57 } $ &$5.82_{- 5.82}^{+62.98}E-05 $ \\
& &$ 1.01_{- 0.23}^{+0.30 } $ & 33.92/ 33&29.09/33&29.06/31& $ 3.92_{-0.51}^{+0.51} $ &$	2.48_{-0.32}^{+0.32} $ &$	2.47_{-0.32}^{+0.32} $  & & & \\  
1116&5 & $2.43_{-0.22}^{+0.24} $ &$4.54_{- 1.58}^{+2.39}E-04 $ &$0.83_{- 0.15}^{+0.18} $ &$2.39_{- 0.32}^{+0.39} $ &$1.12_{- 0.53}^{+0.98}E-03 $ &$0.80_{- 0.15}^{+0.17} $ &$1.19 _{-1.18}^{+1041.89}E-03 $ &$11.33_{- 10.31}^{+2.55} $ &$1.77_{- 1.77}^{+0.33} $ &$4.84_{- 0.47}^{+26.92}E-02 $ \\
& &$ 0.83_{- 0.15}^{+0.18 } $ & 37.53/52&39.93/ 52&36.92/ 50 &  $4.55_{-0.44}^{+0.44} $ &$	3.03_{-0.29}^{+0.29} $ &$	4.05_{-0.39}^{+0.39} $ & & & \\  
1116&6 & $2.76_{-0.18}^{+0.19} $ &$1.02_{- 0.29}^{+0.41}E-03 $ &$1.15_{- 0.16}^{+0.19} $ &$1.98_{- 0.18}^{+0.20} $ &$3.25_{- 1.17}^{+1.82}E-03 $ &$1.14_{- 0.16}^{+0.19} $ &$4.03 _{--1.58}^{+5.81}E-01 $ &$2.04 _{-0.47}^{+47.61} $ &$6.81_{- 3.19}^{+4.19} $ &$1.84_{- 1.84}^{+86.06}E-04 $ \\
& &$ 1.13_{- 0.16}^{+0.18 } $ & 96.25/77&91.86/ 77&90.08/ 75 &  $4.92_{-0.37}^{+0.37} $ &$	3.60_{-0.27}^{+0.27} $ &$	3.75_{-0.28}^{+0.28} $  & & & \\  
1122& 1& $ 1.97_{-0.24}^{+0.25} $ &$ 8.38_{-3.49}^{+5.67}E-05 $ &$ 1.60_{-0.35}^{+0.50}$ & $ 3.57 _{-0.61}^{+0.82}$ & $ 9.82_{-5.53}^{+11.38}E-05$ & $ 1.54_{-0.34}^{+0.48}$ & $ 4.70_{-4.70}^{+9.54}$E-01 & $ 3.28_{-1.01}^{+51.38}$ & $ 6.76_{-6.16}^{+6.17} $ & $ 2.02_{-2.02}^{+22.08}$E-05 \\
& & $ 1.56_{-0.34}^{+0.49}$ & 71.19/ 61& 69.36/ 61& 68.62/ 59& $2.72_{-0.32}^{+0.32} $ &$	1.57_{-0.19}^{+0.19} $ &$	1.62_{-0.19}^{+0.19} $  & & & \\
1122& 2& $ 1.50_{-0.38}^{+0.39} $ &$ 2.33_{-1.41}^{+3.18}E-05 $ &$ 1.30_{-0.42}^{+0.66}$ & $ 5.63 _{-1.76}^{+3.58}$ & $ 1.27_{-1.27}^{+3.90}E-05$ & $ 1.36_{-0.43}^{+0.70}$ & $ 4.16_{-1.52}^{+0.85}$ & $ 1.00_{-1.00}^{+0.00}$ & $ 27.22_{-12.85}^{+32.50 } $ & $ 1.81_{-0.34}^{+5.31}E-04$ \\
& & $ 1.35_{-0.43}^{+0.70}$ & 57.93/ 53& 56.45/ 53& 55.69/ 51& $3.03_{-0.58}^{+0.58} $ &$	1.40_{-0.26}^{+0.26} $ &$	1.43_{-0.27}^{+0.27} $  & & & \\
1122& 3& $ 2.18_{-0.21}^{+0.22} $ &$ 2.24_{-0.77}^{+1.15}E-04 $ &$ 1.12_{-0.19}^{+0.23}$ & $ 2.92 _{-0.39}^{+0.48}$ & $ 3.88_{-1.81}^{+3.21}E-04$ & $ 1.07_{-0.18}^{+0.22}$ & $ 4.22_{-4.22}^{+4.87}E-01$ & $ 2.81_{-0.70}^{+2.07}$ & $ 6.81_{-2.77}^{+3.99} $ & $ 5.24_{-2.83}^{+93.51}E-05$ \\
& & $ 1.09_{-0.19}^{+0.23}$ & 97.95/ 94& 94.09/ 94& 92.28/ 92& $4.18_{-0.39}^{+0.39} $ &$	2.55_{-0.24}^{+0.24} $ &$	2.65_{-0.24}^{+0.24} $  & & & \\
1122& 4& $ 2.11_{-0.53}^{+0.60} $ &$ 9.17_{-9.17}^{+16.78}E-05 $ &$ 1.15_{-0.47}^{+0.83}$ & $ 3.13 _{-1.05}^{+1.86}$ & $ 1.37_{-1.37}^{+5.57}E-04$ & $ 1.10_{-0.45}^{+0.77}$ & $ 8.77_{-8.77}^{+13.14}E-01$ & $ 3.68_{-3.68}^{+399.75 }$ & $ 4.98_{-4.98}^{+191.82} $ & $ 1.17_{-1.17}^{+51.01}E-05$ \\
& & $ 1.13_{-0.46}^{+0.80}$ & 32.80/ 31& 31.87/ 31& 31.38/ 29& $2.05_{-0.50}^{+0.50} $ &$	1.22_{-0.30}^{+0.29} $ &$	1.30_{-0.31}^{+0.31} $ & & & \\
1122& 5& $ 1.98_{-0.40}^{+0.43} $ &$ 7.37_{-4.23}^{+9.07}E-05 $ &$ 1.20_{-0.38}^{+0.62}$ & $ 3.16 _{-0.74}^{+1.15}$ & $ 1.36_{-1.36}^{+2.69}E-04$ & $ 1.18_{-0.37}^{+0.59}$ & $ 1.96_{-0.36}^{+0.37}$ & $ 1.00_{-1.00}^{+-1.00}$ & $ 2.81_{-2.81}^{+77.88 } $ & $ 5.51_{-1.02}^{+5064.47}E-05$ \\
& & $ 1.18_{-0.37}^{+0.58}$ & 40.29/ 43& 36.93/ 43& 36.42/ 41& $2.36_{-0.45}^{+0.45} $ &$	1.27_{-0.24}^{+0.24} $ &$	1.15_{-0.21}^{+0.21} $  & & & \\
1122& 6& $ 1.80_{-0.30}^{+0.32} $ &$ 1.07_{-0.51}^{+0.92}E-04 $ &$ 0.98_{-0.24}^{+0.31}$ & $ 4.01 _{-0.95}^{+1.53}$ & $ 1.10_{-0.76}^{+1.96}E-04$ & $ 0.93_{-0.23}^{+0.30}$ & $ 7.20_{-7.20}^{+157.21}E-02$ & $ 15.14_{-12.49}^{+-15.14 }$ & $ 2.38_{-2.38}^{+7.66} $ & $ 3.52_{-3.51}^{+2374.97}E-05$ \\
& & $ 0.97_{-0.24}^{+0.31}$ & 50.81/ 53& 52.36/ 53& 50.71/ 51& $5.62_{-0.77}^{+0.77} $ &$	2.89_{-0.40}^{+0.40} $ &$	4.97_{-0.68}^{+0.68} $  & & & \\
1124&1 & $2.67_{-0.38}^{+0.43} $ &$2.52_{-1.24}^{+2.55}E-04 $ &$0.97_{-0.26}^{+0.36} $ &$2.21_{-0.45}^{+0.57} $ &$5.85_{-3.63}^{+9.83}E-04 $ &$0.93_{-0.25}^{+0.34} $ &$3.64_{-3.64}^{+7.06}E-01 $ &$2.35_{-0.81}^{+ 20.35} $ &$6.34_{-5.07}^{+8.07} $ &$4.75_{-4.75}^{+210.83}E-05 $ \\
& &$0.95_{-0.25}^{+0.35 } $ & 52.36 /40 &50.16/40& 49.02/38&$  1.47_{-0.23}^{+0.23} $ &$	1.10_{-0.17}^{+0.17} $ &$	1.15_{-0.17}^{+0.17} $  & & & \\
1124&2 & $2.90_{-0.38}^{+0.43} $ &$4.58_{-2.27}^{+4.62} E-04$ &$0.94_{-0.25}^{+0.33} $ &$1.83_{-0.32}^{+0.41} $ &$1.60_{-0.96}^{+2.32}E-03 $ &$0.97_{-0.25}^{+0.34} $ &$3.74_{-3.74}^{+10.37}E-01 $ &$1.85_{-0.51}^{+ 71.82} $ &$7.24_{-7.24}^{+ 10.27 } $ &$8.06 _{-8.06}^{+383.74}E-05 $ \\
& &$0.96 _{-0.25 }^{+0.34} $ &35.96/ 51 & 33.64/51&33.31/49 &$1.67_{-0.25}^{+0.25} $ &$	1.24_{-0.18}^{+0.18} $ &$	1.28_{-0.19}^{+0.19} $  & & & \\ 
1124&3 & $1.98_{-0.56}^{+0.61} $ &$5.63_{-5.63}^{+11.10}E-05 $ &$1.13_{-0.41}^{+0.64} $ &$2.64_{-0.79}^{+1.82} $ &$2.00_{-2.00}^{+6.92}E-04 $ &$1.12_{-0.42}^{+0.67} $ &$1.13_{- 0.62}^{+3.41}E+01 $ &$ 1.00_{-0.55}^{+ 0.00} $ &$99.69_{-39.31}^{+79.85} $ &$2.60_{- 0.55}^{+121.17}E-03 $ \\
& &$1.12_{- 0.40}^{+0.60 } $& 67.54 /63 &69.93/63& 64.11/61&$  1.78_{-0.39}^{+0.39} $ &$	0.84_{-0.19}^{+0.19} $ &$	4.01_{-0.85}^{+0.85} $  & & & \\
1124&4 & $2.69_{-0.49}^{+0.58} $ &$2.56_{-1.55}^{+4.15}E-04 $ &$1.52_{-0.50}^{+0.86} $ &$2.24_{-0.52}^{+0.74} $ &$5.11_{-5.11}^{+11.89}E-04 $ &$1.59_{-0.52}^{+0.92} $ &$<1.00E-03$ &$2.04_{-0.62}^{+0.52} $ &$7.87_{-7.87}^{+ 4.58} $ &$3.60_{-0.68}^{+18804.60}E-03 $ \\
& &$1.59_{-0.51}^{+0.91} $ &27.07/26 &25.25/26 & 25.03/24 &$ 1.45_{-0.28}^{+0.28} $ &$	1.01_{-0.19}^{+0.19} $ &$	1.03_{-0.20}^{+0.20} $  & & & \\ 
1124&5 & $2.39_{-0.27}^{+0.29} $ &$2.68_{-1.12}^{+1.90}E-04 $ &$1.04_{-0.21}^{+0.26} $ &$2.48_{-0.38}^{+0.48} $ &$5.92_{-3.12}^{+6.33}E-04 $ &$1.06_{-0.21}^{+0.26} $ &$3.79_{-3.79}^{+5.65}E-01 $ &$2.72_{-0.88}^{+77.85} $ &$ 5.98_{-5.76}^{+5.19} $ &$6.01_{-6.00}^{+210.74}E-05 $ \\
& &$1.05 _{-0.21 }^{+0.26 } $& 52.44/41 &52.69/41& 50.78/39&$3.01_{-0.33}^{+0.33} $ &$	1.88_{-0.21}^{+0.21} $ &$	2.04_{-0.22}^{+0.22} $ & & & \\ 
1124&6 & $2.75_{-0.26}^{+0.28} $ &$5.03_{-2.02}^{+3.30}E-04 $ &$1.85_{-0.37}^{+0.53} $ &$1.85_{-0.23}^{+0.28} $ &$2.23_{-1.09}^{+2.07}E-03 $ &$1.83_{-0.36}^{+0.52} $ &$6.20_{-6.20}^{+1.56}E-01 $ &$138.66_{-137.66}^{+133.5} $ &$7 0.02_{-0.02}^{+4.23} $ &$8.71_{- 4.19}^{+ 1728.93}E-07 $ \\
& &$1.85_{- 0.37}^{+ 0.53 } $ &67.39 /62 &70.80/62 & 67.26/60 &$2.49_{-0.25}^{+0.25} $ &$	1.78_{-0.18}^{+0.18} $ &$	2.32_{-0.23}^{+0.23} $  & & & \\
1157& 1& $ 2.34_{-0.10}^{+0.10} $ &$ 7.09_{-1.24}^{+1.48}E-04 $ &$ 1.00_{-0.09}^{+0.10}$ & $ 2.61 _{-0.17}^{+0.18}$ & $ 1.42_{-0.35}^{+0.46}E-03$ & $ 1.02_{-0.09}^{+0.10}$ & $ 3.18_{-3.18}^{+5.40}E-01$ & $ 2.51_{-0.36}^{+0.55}$ & $ 7.04_{-1.47}^{+1.92} $ & $ 1.85_{-1.06}^{+30.46}E-04$ \\
& & $ 1.01_{-0.09}^{+0.10}$ & 141.18/ 102& 113.85/ 102& 110.37/ 100& $8.82_{-0.42}^{+0.42} $ &$	5.70_{-0.27}^{+0.27} $ &$	5.91_{-0.27}^{+0.28} $  & & & \\
1157& 2& $ 2.40_{-0.10}^{+0.11} $ &$ 8.13_{-1.48}^{+1.79}E-04 $ &$ 1.03_{-0.09}^{+0.10}$ & $ 2.61 _{-0.18}^{+0.19}$ & $ 1.48_{-0.39}^{+0.52}E-03$ & $ 1.02_{-0.09}^{+0.10}$ & $ 3.62_{-3.62}^{+3.62}E-01$ & $ 3.34_{-0.67}^{+1.34}$ & $ 5.02_{-1.34}^{+1.35} $ & $ 1.62_{-0.93}^{+81.15}E-04$ \\
& & $ 1.02_{-0.09}^{+0.10}$ & 122.14/ 110& 125.54/ 110& 108.40/ 108& $8.80_{-0.42}^{+0.42} $ &$	5.89_{-0.28}^{+0.28} $ &$	6.51_{-0.31}^{+0.31} $ & & & \\
1157& 3& $ 2.19_{-0.08}^{+0.08} $ &$ 7.34_{-1.08}^{+1.25}E-04 $ &$ 1.09_{-0.08}^{+0.09}$ & $ 2.89 _{-0.16}^{+0.17}$ & $ 1.31_{-0.28}^{+0.35}E-03$ & $ 1.09_{-0.08}^{+0.09}$ & $ 1.13_{-0.11}^{+0.12}$ & $ 154.39 _{-153.39 }^{+32.59}$ & $ 0.01_{-0.01}^{+3.91} $ & $ 1.46_{-0.25}^{+77.45}E-06$ \\
& & $ 1.08_{-0.08}^{+0.09}$ & 193.43/ 150& 154.50/ 150& 147.82/ 148& $13.40_{-0.53}^{+0.53} $ &$	8.24_{-0.32}^{+0.32} $ &$	9.95_{-0.39}^{+0.39} $  & & & \\
1157& 4& $ 2.23_{-0.11}^{+0.11} $ &$ 7.58_{-1.46}^{+1.79}E-04 $ &$ 1.04_{-0.11}^{+0.12}$ & $ 2.91 _{-0.21}^{+0.23}$ & $ 1.25_{-0.34}^{+0.45}E-03$ & $ 0.99_{-0.10}^{+0.11}$ & $ 8.19_{-8.19}^{+4.04}E-01$ & $ 2.63_{-0.48}^{+1.98}$ & $ 7.11_{-3.92}^{+3.68} $ & $ 1.15_{-0.58}^{+8.88}E-04$ \\
& & $ 0.99_{-0.10}^{+0.11}$ & 126.83/ 79& 87.77/ 79& 87.32/ 77& $12.50_{-0.67}^{+0.67} $ &$	8.17_{-0.43}^{+0.43} $ &$	8.20_{-0.43}^{+0.43} $ & & & \\
1157& 5& $ 2.30_{-0.10}^{+0.10} $ &$ 7.80_{-1.34}^{+1.60}E-04 $ &$ 1.10_{-0.10}^{+0.11}$ & $ 2.75 _{-0.18}^{+0.20}$ & $ 1.39_{-0.35}^{+0.45}E-03$ & $ 1.09_{-0.10}^{+0.11}$ & $ 2.52_{-2.52}^{+6.95}E-01$ & $ 2.88_{-0.49}^{+0.87}$ & $ 6.19_{-1.45}^{+1.73} $ & $ 2.47_{-2.47}^{+26.32}E-04$ \\
& & $ 1.09_{-0.10}^{+0.11}$ & 130.00/ 102& 116.22/ 102& 110.27/ 100& $10.90_{-0.51}^{+0.51} $ &$	7.05_{-0.33}^{+0.33} $ &$	7.45_{-0.35}^{+0.35} $  & & & \\
1253& 1& $ 1.48_{-0.13}^{+0.13} $ &$ 1.58_{-0.37}^{+0.48}E-04 $ &$ 0.91_{-0.11}^{+0.12}$ & $ 5.40 _{-0.72}^{+0.93}$ & $ 1.08_{-0.45}^{+0.69}E-04$ & $ 0.90_{-0.11}^{+0.12}$ & $ 1.23_{-0.35}^{+0.30}$ & $ 500.00 _{-499.00 }^{+-500.00}$ & $ 0.04_{-0.04}^{+1.94} $ & $ 3.85_{-0.74}^{+377.69}E-07$ \\
& & $ 0.90_{-0.11}^{+0.12}$ & 64.62/ 67& 63.22/ 67& 59.87/ 65& $22.00_{-1.38}^{+1.38} $ &$	10.00_{-0.63}^{+0.63} $ &$	17.70_{-1.11}^{+1.11} $ & & & \\
1253& 3& $ 1.45_{-0.14}^{+0.15} $ &$ 1.23_{-0.36}^{+0.48}E-04 $ &$ 1.32_{-0.20}^{+0.25}$ & $ 6.00 _{-0.99}^{+1.34}$ & $ 6.31_{-3.14}^{+5.55}E-05$ & $ 1.29_{-0.19}^{+0.24}$ & $ <1.00E-03$ & $ 5.61_{-1.70}^{+0.86}$ & $ 5.89_{-1.89}^{+0.67} $ & $ 8.78_{-0.65}^{+7.84}E-04$ \\
& & $ 1.30_{-0.19}^{+0.24}$ & 81.83/ 69& 79.28/ 69& 78.52/ 67& $18.80_{-1.40}^{+1.40} $ &$	9.09_{-0.68}^{+0.68} $ &$	10.10_{-0.75}^{+0.75} $  & & & \\
1253& 4& $ 1.53_{-0.23}^{+0.24} $ &$ 1.73_{-0.70}^{+1.14}E-04 $ &$ 1.52_{-0.33}^{+0.38}$ & $ 5.60 _{-1.44}^{+2.66}$ & $ 9.16_{-6.70}^{+17.30}E-05$ & $ 1.46_{-0.33}^{+0.38}$ & $ <1.00E-03$ & $ 21.68_{-14.33}^{+12.39}$ & $ 2.54_{-2.11}^{+1.14} $ & $ 3.64_{-0.38}^{+21.03}E-04$ \\
& & $ 1.52_{-0.33}^{+0.37}$ & 24.09/ 21& 34.17/ 21& 24.09/ 19& $20.50_{-2.14}^{+2.14} $ &$	9.85_{-1.05}^{+1.05} $ &$	20.20_{-2.10}^{+2.10} $ & & & \\
1253& 5& $ 1.58_{-0.16}^{+0.17} $ &$ 1.70_{-0.49}^{+0.66}E-04 $ &$ 1.75_{-0.30}^{+0.35}$ & $ 4.92 _{-0.74}^{+0.96}$ & $ 1.37_{-0.64}^{+1.08}E-04$ & $ 1.69_{-0.29}^{+0.33}$ & $ 1.14_{-1.14}^{+0.73}$ & $ 3.89_{-1.34}^{+33.63}$ & $ 6.53_{-6.39}^{+8.60} $ & $ 4.52_{-4.52}^{+33.14}E-05$ \\
& & $ 1.66_{-0.29}^{+0.33}$ & 41.15/ 32& 27.86/ 32& 27.07/ 30& $17.30_{-1.55}^{+1.56} $ &$	8.56_{-0.75}^{+0.75} $ &$	8.30_{-0.73}^{+0.73} $  & & &\\
1267& 1& $ 2.42_{-0.13}^{+0.14} $ &$ 4.93_{-1.08}^{+1.38}E-04 $ &$ 1.12_{-0.12}^{+0.14}$ & $ 2.53 _{-0.21}^{+0.23}$ & $ 9.90_{-3.06}^{+4.38}E-04$ & $ 1.10_{-0.12}^{+0.14}$ & $ 4.19_{-4.19}^{+4.00}E-01$ & $ 2.89_{-0.60}^{+1.49}$ & $ 5.70_{-1.76}^{+1.96} $ & $ 9.15_{-5.32}^{+326.12}E-05$ \\
& & $ 1.11_{-0.12}^{+0.14}$ & 74.06/ 83& 69.33/ 83& 62.26/ 81& $5.11_{-0.29}^{+0.29} $ &$	3.42_{-0.20}^{+0.20} $ &$	3.67_{-0.21}^{+0.21} $  & & & \\
1267& 2& $ 2.42_{-0.12}^{+0.13} $ &$ 5.62_{-1.17}^{+1.46}E-04 $ &$ 0.91_{-0.10}^{+0.12}$ & $ 2.56 _{-0.19}^{+0.21}$ & $ 1.07_{-0.30}^{+0.42}E-03$ & $ 0.94_{-0.10}^{+0.12}$ & $ 6.08_{-6.08}^{+4.40}E-01$ & $ 2.22_{-0.34}^{+0.81}$ & $ 8.29_{-3.49}^{+3.52} $ & $ 8.41_{-3.19}^{+93.64}E-05$ \\
& & $ 0.94_{-0.10}^{+0.12}$ & 118.77/ 82& 81.23/ 82& 80.72/ 80& $5.77_{-0.34}^{+0.34} $ &$	3.92_{-0.23}^{+0.23} $ &$	3.93_{-0.23}^{+0.23} $  & & & \\
1267& 3& $ 2.20_{-0.12}^{+0.13} $ &$ 3.68_{-0.78}^{+0.98}E-04 $ &$ 1.09_{-0.12}^{+0.13}$ & $ 2.88 _{-0.23}^{+0.26}$ & $ 6.42_{-1.88}^{+2.60}E-04$ & $ 1.07_{-0.11}^{+0.13}$ & $ 3.85_{-3.85}^{+4.74}E-01$ & $ 2.68_{-0.46}^{+0.86}$ & $ 7.10_{-1.90}^{+2.77} $ & $ 9.13_{-4.52}^{+122.89}E-05$ \\
& & $ 1.07_{-0.11}^{+0.13}$ & 111.99/ 101& 99.53/ 101& 97.13/ 99& $6.54_{-0.36}^{+0.36} $ &$	3.99_{-0.22}^{+0.22} $ &$	4.12_{-0.23}^{+0.23} $  & & & \\
1267& 4& $ 2.71_{-0.19}^{+0.20} $ &$ 7.97_{-2.48}^{+3.58}E-04 $ &$ 1.25_{-0.18}^{+0.21}$ & $ 2.12 _{-0.21}^{+0.25}$ & $ 2.02_{-0.80}^{+1.29}E-03$ & $ 1.23_{-0.18}^{+0.21}$ & $ 3.46_{-3.46}^{+5.43}E-01$ & $ 2.97_{-1.03}^{+19.59}$ & $ 4.69_{-3.67}^{+3.15} $ & $ 1.43_{-1.43}^{+101.67}E-04$ \\
& & $ 1.24_{-0.18}^{+0.21}$ & 40.73/ 42& 41.84/ 42& 36.84/ 40& $4.31_{-0.33}^{+0.33} $ &$	3.10_{-0.24}^{+0.24} $ &$	3.43_{-0.27}^{+0.27} $  & & & \\
1267& 5& $ 2.28_{-0.13}^{+0.14} $ &$ 4.25_{-1.00}^{+1.29}E-04 $ &$ 0.95_{-0.12}^{+0.13}$ & $ 2.88 _{-0.24}^{+0.27}$ & $ 6.63_{-2.10}^{+3.01}E-04$ & $ 0.94_{-0.11}^{+0.13}$ & $ 2.54_{-2.54}^{+9.81}E-01$ & $ 2.29_{-0.34}^{+0.49}$ & $ 9.35_{-2.52}^{+5.09} $ & $ 1.10_{-0.69}^{+15.89}E-04$ \\
& & $ 0.94_{-0.12}^{+0.13}$ & 81.71/ 65& 48.29/ 65& 47.81/ 63& $6.27_{-0.41}^{+0.41} $ &$	4.10_{-0.26}^{+0.26} $ &$	4.04_{-0.26}^{+0.26} $ & & & \\ 
\end{longtable}
\end{center}
\end{landscape}

